A Continual and Incremental Learning Approach for TinyML On-device Training Using Dataset Distillation and Model Size Adaption

A new algorithm for incremental learning in the context of Tiny Machine learning (TinyML) is presented, which is optimized for low-performance and energy efficient embedded devices. TinyML is an emerging field that deploys machine learning models on resource-constrained devices such as microcontrollers, enabling intelligent applications like voice recognition, anomaly detection, predictive maintenance, and sensor data processing in environments where traditional machine learning models are not feasible. The algorithm solve the challenge of catastrophic forgetting through the use of knowledge distillation to create a small, distilled dataset. The novelty of the method is that the size of the model can be adjusted dynamically, so that the complexity of the model can be adapted to the requirements of the task. This offers a solution for incremental learning in resource-constrained environments, where both model size and computational efficiency are critical factors. Results show that the proposed algorithm offers a promising approach for TinyML incremental learning on embedded devices. The algorithm was tested on five datasets including: CIFAR10, MNIST, CORE50, HAR, Speech Commands. The findings indicated that, despite using only 43% of Floating Point Operations (FLOPs) compared to a larger fixed model, the algorithm experienced a negligible accuracy loss of just 1%. In addition, the presented method is memory efficient. While state-of-the-art incremental learning is usually very memory intensive, the method requires only 1% of the original data set.

==> Archiv/1Intro2.tex <==
\section{Introduction} 

TinyML, also known as ultra-low power machine learning, is a subfield of artificial intelligence (AI) that focuses on the development of machine learning (ML) models that can run on extremely low-power and resource-constrained devices. The goal of TinyML is to enable the deployment of sophisticated AI algorithms on small, inexpensive, and low-power devices, such as IoT sensors, wearables, and smart embedded systems.

The advantages of machine learning close to the data source are \cite{Ren.15.03.2021}: 


\begin{itemize}
\item \textbf{Data security}: Since less information needs to be shared with external entities, data security and privacy can be better ensured. 
\item \textbf{Latency}: Data transmission takes time and is often associated with a delay. When this process is eliminated, the result is available immediately. 
\item \textbf{Energy saving and cost}: If a DNN has to be retrained in the cloud, there is a high overhead in energy costs for sending and receiving the DNN. however, if the DNN is only executed, the energy consumption for communication may be higher than training the DNN locally.
\item \textbf{Connection availability}: If the device relies on the internet to function and the connection to the internet is interrupted, data cannot be sent to the server. This for example happens, if you try to use a voice assistant and it does not respond, because it is not connected to the internet.
\end{itemize}


The field of training models on embedded devices is a rapidly emerging area of research, leading to various innovations and applications. However, it should also be noted that this approach comes with its own set of limitations. In contrast to utilizing cloud servers, embedded systems, such as Micro-Controller Units (MCUs), tend to be highly constrained in terms of resources. Typical limitations of these embedded devices include limited device memory or limited computing power.



Given the constrained memory capacity of embedded devices, it is often infeasible to store a large data set, rendering traditional post-training techniques impractical. As such, there is a need for the incorporation of incremental or continuous learning strategies. 
continuous learning, also known as lifelong learning, is a type of machine learning that enables models to acquire and retain knowledge incrementally across a prolonged period of time, and to learn from a variety of tasks without forgetting previous knowledge. Continuous learning differs from incremental learning in that it focuses on learning new situations, such as a data drift, while incremental learning focuses on learning new classes. One of the main challenges of continuous learning is the phenomenon of catastrophic forgetting, which refers to the rapid and drastic degradation of the performance of a model on previously learned tasks as it is trained on new tasks.

However, many existing incremental and continuous learning methods are excessively memory-intensive.

This paper suggests a novel approach for enabling scalable and computationally efficient incremental learning on embedded devices. Our proposed algorithm facilitates the continuous training of models on-device and enables the adoption of model size as the data necessitates. This approach has the added benefit of allowing for the initial deployment of a compact model, thus conserving both memory and computational resources, which can be incrementally expanded as needed.  The incremental learning approach is implemented as a knowledge distillation technique. We have tested the method on 5 different data sets, including: CIFAR10, MNIST, CORE50, HAR, Speech Commands. Using only 1\% of the memory of the dataset and only 43\% of the FLOPs of the baseline, we were able to train models that have only 1\% points of accuracy loss compared to training with the whole dataset. 



The code for the algorithm is written in Python and is directly usable and available on GitHub: [Link einfügen]





==> Archiv/2Related2.tex <==
\iffalse
\begin{figure*}[!hbt] 
	\centering
	\includegraphics[width=0.9\textwidth]{figures/Flow.png} 
	\caption{The steps that are carried out with TinyProp. 1. the forward pass is performed. 2. the loss function is calculated and the local error is summed up 3. the local k for this layer is determined from the summed error. 4. the top k gradients are searched for. 5. the sparse backpropagation algorithm is performed.}
	\label{tinyprop}
\end{figure*}
\fi


\section{related work}
\subsection{Incremental Learning}

CL approaches can be broadly divided into three main topics: Regularization-based approaches preserve learning from previous tasks through regularization terms placed on model weights (EWC\cite{Kirkpatrick.2017}, synaptic intelligence \cite{pmlr-v70-zenke17a}), structural regularization \cite{JoanSerra.2018}, or functional regularization \cite{Cha.12.06.2020}\cite{pmlr-v162-rudner22a}). In other work, incremental momentum matching \cite{Lee.2017} proposes a model merging step where a model trained for the new task is merged with the model trained for the previous tasks, or knowledge distillation based regularization \cite{Li.2018} is used to preserve the learning from the previous tasks. Architectural adaptations modify model architectures to address CL challenges, such as using a recurrent neural network \cite{Cossu.71920207242020}, learning from overcapacitated deep neural networks in an adaptive manner that repeatedly compresses sparse connections \cite{SOKAR20211}, or using overlapping convolutional filters \cite{NEURIPS2019_3b220b43}. Other work attempts to identify common information across tasks (CLAW \cite{Adel.21.11.2019}) using variational inference. Replay-based approaches preserve knowledge about previous tasks by storing a small memory buffer of representative data samples from previous tasks for further training alongside new tasks (ER \cite{ROBINS.1995}). Some approaches add a distillation loss to preserve learned representations (iCaRL \cite{Rebuffi.23.11.2016}) or classifier outputs (DER \cite{NEURIPS2020_b704ea2c} ) for points in the buffer. Gradient Episodic Memory (GEM) \cite{LopezPaz.2017}, AGEM) \cite{Chaudhry.02.12.2018}) focuses on minimizing catastrophic forgetting through efficient use of episodic memory. Meta-Experience Replay (MER) \cite{Riemer.29.10.2018} inserts a penalty term for inter-task interference into a meta-learning framework. Maximally Interfered Retrieval (MIR) \cite{Aljundi.2019} uses controlled memory samples for the replay buffer by retrieving samples that will be most negatively affected by the likely update of model parameters. Of these approaches, distillation losses in the replay buffer \cite{Rebuffi.23.11.2016} \cite{NEURIPS2020_b704ea2c} show the strongest performance gains on standard CL benchmarks. Coreset selection: Coresets \cite{Ros.2020} are small, informative, weighted data subsets that approximate certain attributes (e.g., loss, gradients, logits) of the original data. Previous work \cite{HarPeled.2004}\cite{Lemke.2016} used coresets for unsupervised learning problems such as K-means and K-medians clustering. Coresets enable efficient and scalable Bayesian inference \cite{JackyZhang.2021}\cite{Campbell.2019}\cite{Campbell.07.06.2019}\cite{TrevorCampbell.2018} by approximating the logit sum of the model for the entire data. Several recent works \cite{Killamsetty.2021}\cite{Mirzasoleiman.2020}\cite{BaharanMirzasoleiman.2020}\cite{Killamsetty.2021b}\cite{KrishnatejaKillamsetty.2021} also use coresets to approximate the gradient sum of individual samples over the entire dataset to enable efficient and robust supervised learning. Although coresets are increasingly used in supervised and unsupervised learning scenarios, the problem of coreset selection for CL is relatively under-researched. In the following, we discuss existing coreset-based approaches for CL.


Coresets for Replay-based CL: Approaches include selecting replay buffers by maximizing criteria such as sample gradient diversity (GSS \cite{Aljundi.2019}), a mixture of mini-batch gradient similarity and cross-batch diversity (OCS \cite{Yoon.02.06.2021}), Adversarial Shapley Value (ASER \cite{Shim.31.08.2020}), or Representation Matching (iCARL \cite{Rebuffi.23.11.2016}). These approaches introduce a secondary selection criterion (to reduce interference from the current task and forgetting of previous tasks) that is very specific to each approach. As a result, they cannot be generalized for different CL loss criteria. Moreover, previous approaches have not considered the weighted selection of replay buffers, which increases the representation possibilities of replay buffers. The closest to our work is a recent paper \cite{NEURIPS2020_aa2a7737}, which proposes to solve a two-stage optimization to select the optimal rendition buffer under certain assumptions rather than for a specific loss function. Their proposal is computationally expensive, intractable in scenarios with large tasks, and scales poorly with buffer size; furthermore, no comparison has been made with recent strong proposals \cite{NEURIPS2020_b704ea2c}. In our experiments, we compare directly with this approach. 

\begin{figure*}[!hbt] 
	\centering
	\includegraphics[width=0.9\textwidth]{figures/flowincrement.png} 
	\caption{The graph displays the steps involved in tinyML incremental learning. The process begins with distilling data to decrease the size of the dataset, making it more manageable for embedded devices. This distilled dataset is then used to train the neural network. Once the training is complete, the model's accuracy is evaluated to determine if it meets the desired threshold. If the accuracy is not satisfactory, the model complexity is increased to enhance its performance. Finally, new data is collected, and the process repeats, allowing the model to continuously learn and improve.}
	\label{tinyprop}
\end{figure*}

\subsection{Dataset distilation}
Wang et al. [44] pioneered dataset distillation by proposing to define model weights as a function of the distilled pictures and improve them using gradient-based hyperparameter optimization [23], which is also frequently utilized in meta-learning research [8, 27]. Following that, various studies enhanced the results by learning soft labels [2, 38], amplifying the learning signal by gradient fitting [47], including augmentations [45], and optimizing with regard to the infinite width kernel boundary [25, 26]. Dataset distillation has facilitated a variety of applications, including continuous learning [44, 45, 47].
For photos, text, and medical image data, efficient neural architecture search [45, 47], federated learning [11, 37, 50], and privacy-friendly ML [22, 37] are used.Our technique, as stated in the introduction, does not rely on single-step behavioral matching [45, 47], expensive unrolling of full optimization trajectories [38, 44], or large-scale neural tangent kernel calculations [25, 26]. Instead, our strategy facilitates broad-scale trajectory modification by transferring information from pre-trained specialists.
In contrast to our work, Zhao and Bilen's [46] technique ignores the optimization phases entirely, instead focusing on distribution matching between synthetic and actual data. While this approach is suitable to higher resolution datasets (e.g., Tiny ImageNet), it performs worse in most circumstances since it uses less RAM (e.g., compared to previous work [45, 47]). On both conventional benchmarks and higher resolution datasets, our strategy simultaneously decreases storage costs while outperforming earlier work [45, 47] and the concurrent method [46]. A similar area of study employs generative models to generate training data [24, 36]. However, because such approaches do not produce a tiny dataset, they cannot be directly compared to dataset distillation methods. 





Method:
%Once the neural network has been trained, it can be used for the application. New data can be stored to improve the network's performance and adapt it to new conditions. However, if the network is re-trained with new data and the accuracy of the model drops, the neural network can be scaled up to restore accuracy. This step is particularly useful for embedded devices, as it is not necessary to use a large neural network from the beginning, which in turn saves memory and computational resources.
%The whole process is shown in Figure 1.
%In our approach, the network never actually sees the real data. Instead, we distil out of the current data $\mathcal{X}_t$ and generate a set of distilled data $\mathcal{X}_t^\prime$ such that $|\mathcal{X}_t^\prime|\ll|\mathcal{X}_t|$ for each $t$ and with (ideally) similar training performance. The neural network is then trained on the distilled data $\{\mathcal{X}_t^\prime\}_{i=1}^t$ at step $t$ and is evaluated on $\{\mathcal{T}_t\}_{t=1}^n$. 

==> Archiv/5result2.tex <==

\begin{figure*}[!hbt] 
	\centering
	\includegraphics[width=0.9\textwidth]{figures/SCMnist.png} 
	\caption{The steps that are carried out with TinyProp. 1. the forward pass is performed. 2. the loss function is calculated and the local error is summed up 3. the local k for this layer is determined from the summed error. 4. the top k gradients are searched for. 5. the sparse backpropagation algorithm is performed.}
	\label{ab}
\end{figure*}



\begin{figure*}[!hbt] 
	\centering
	\includegraphics[width=0.9\textwidth]{figures/cifar core 50.png} 
	\caption{The steps that are carried out with TinyProp. 1. the forward pass is performed. 2. the loss function is calculated and the local error is summed up 3. the local k for this layer is determined from the summed error. 4. the top k gradients are searched for. 5. the sparse backpropagation algorithm is performed.}
	\label{ba}
\end{figure*}

\subsection{Results}
The results of the above-mentioned experiments show that the presented method of incremental learning can be used to perform computations efficiently. The technique saves capacity at two points. The first is through an incremental approach, which is memory efficient since only a small fraction of the data set is stored. The second is that the model can grow with the task and therefore initially requires fewer resources in terms of computing and storage capacity.



\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over steps & Needed FLOPs & average Needed Memory over time\\
Baseline                & 85.4 \%        & 47.8 \%                      & 100 \%       & 500 mb\\
Largest model           & 57.7 \%        & 35.6 \%                      & 100 \%       & 500 mb \\
Adaptive Model          & 58.2 \%        & 35.9 \%                      & 43\%       & 500 mb\\
Catastrophic Forgotting & 10 \%        & 10 \%                      & 100 \%       & 500 mb        
\end{tabular}%
}
\caption{CIFAR10 }
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs & Needed Memory over time \\
Baseline                & 55.3 \%        & 36.5 \%                      & 100 \%       & 500 mb                  \\
Largest model           & 44.2 \%        & 28.9 \%                      & 100 \%       & 500 mb                  \\
Adaptive Model          & 43.2 \%        & 26.1 \%                      & 49\%       & 500 mb                  \\
Catastrophic Forgotting & 3.7 \%        & 3.6 \%                      & 100 \%       & 500 mb                 
\end{tabular}%
}
\caption{CORE50 }
\label{tab:my-table}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs & Needed Memory over time \\
Baseline                & 95 \%        & 45.6 \%                      & 100 \%       & 500 mb                  \\
Largest model           & 70.8 \%        & 35 \%                      & 100 \%       & 500 mb                  \\
Adaptive Model          & 70.4 \%        & 33.7 \%                      & 36 \%       & 500 mb                  \\
Catastrophic Forgotting & 3.8 \%        & 2.9 \%                      & 100 \%       & 500 mb                 
\end{tabular}%
}
\caption{Spechcommands }
\label{tab:my-table}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs & Needed Memory over time \\
Baseline                & 98.8 \%        & 78.8 \%                      & 100 \%       & 500 mb                  \\
Largest model           & 92.7 \%        & 76.9 \%                      & 100 \%       & 500 mb                  \\
Adaptive Model          & 92.8 \%        & 76.1 \%                      & 36\%       & 500 mb                  \\
Catastrophic Forgotting & 60.1 \%        & 66.2 \%                      & 100 \%       & 500 mb                 
\end{tabular}%
}
\caption{MNIST }
\label{tab:my-table}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs & Needed Memory over time \\
Baseline                & 83.1 \%        & 43.1 \%                      & 100 \%       & 500 mb                  \\
Largest model           & 65.1 \%        & 37.3 \%                      & 100 \%       & 500 mb                  \\
Adaptive Model          & 64.4 \%        & 36.9 \%                      & 36\%       & 500 mb                  \\
Catastrophic Forgotting & 15 \%        & 12.5 \%                      & 100 \%       & 500 mb                 
\end{tabular}%
}
\caption{HAR }
\label{tab:my-table}
\end{table}



\subsubsection{Incremental learning}
Mit der Vorgestellten technik lässt sich wie die experimente zeigen inkremental learning erfolgreich durchführen. Der Vorteil daran destilierte Datensätze zu verwenden zeigt sich an den geringen overhead an speicher der benötigt wird um gegen katastrophic forgetting vorzugehen.



\subsubsection{Effitients der Adaptiven Model größe}
A novelty of our technology is that the models can be expanded. By enlarging the models only when needed, instead of using a large model from the beginning, we save memory and computational resources. For example, our experiments have shown that with an adaptive model we only need 36\% of the FLOPS over the whole training process for speech commands and HAR, compared to a fixed model. With CIFAR10 we always need only 43\% of the FLOPs and even with a heavy data set like CORE50 we need only 49\% of the FLOPs. This saving is directly related to the energy saving and time saving. The experiments also show that the accuracy has little or no loss despite the large savings. Thus, in the best case, the CIFAR10 data set has a better average accuracy of 0.3 \% and the CORE50 data set has only an average loss of 2.8 \% accuracy over the whole training process.






==> Archiv/5results2.tex <==


\section{Results and Discussion}

In this section, we delve into the findings obtained from our experimentation on five diverse datasets: CIFAR10, CORe50, Speech Commands, MNIST, and HAR. These results elucidate the successful implementation and benefits of the incremental learning approach proposed in this study, mainly focusing on memory efficiency and computational savings.

\subsection{Incremental Learning and Memory Efficiency}

Our experiments demonstrated the successful application of the incremental learning technique, especially in the context of on-device training where memory limitations are often a hindrance. The use of distilled datasets proved beneficial in combating the challenge of catastrophic forgetting typically associated with continuous learning. Remarkably, the memory overhead required for this technique was a mere 1\% of the total size of the original dataset. This reveals the potential of our proposed method in situations where device memory is a significant concern.

\subsection{Efficiencies of the Adaptive Model Size}

A unique aspect of our method is the adaptive expansion of our models, which helps to alleviate the demands on memory and computational resources. By incrementally increasing the model size as per the task requirements, we could avoid deploying an overly large model from the outset.

When examining the FLOPs required across the training process, our method demonstrated considerable savings. In the Speech Commands and HAR datasets, we only utilized 36\% of the FLOPs required by a fixed model. For the CIFAR10 dataset, this requirement dropped to 43\%, and even for the computationally heavy CORe50 dataset, our method needed only 49\% of the FLOPs. These reductions directly correlate with energy and time savings, making our technique particularly valuable for on-device training where these resources are scarce.

Further, our results showed minimal, if any, sacrifice in accuracy despite these significant savings. On average, the CIFAR10 dataset experienced a slight 0.3\% improvement in accuracy over the entire training process, while the CORe50 dataset recorded a marginal average loss of 2.8\% in accuracy. These outcomes suggest that the proposed method offers an effective balance between resource utilization and model performance.

\subsection{Performance Comparison}

Upon comparing the performance of the baseline model, largest model, adaptive model, and a model with catastrophic forgetting, the efficiency and effectiveness of our approach became even more evident.

\begin{table}[h!]
\centering
\begin{tabular}{lllll}
\hline
Model & End accuracy & Average accuracy over steps & Needed FLOPs \
\hline
Baseline & 85.4\% & 47.8\% & 100\% \
Largest model & 57.7\% & 35.6\% & 100\% \
Adaptive Model (ours) & 58.2\% & 35.9\% & 43\% \
Catastrophic forgetting & 10\% & 10\% & 100\% \
\hline
\end{tabular}
\caption{Performance comparison on CIFAR10 dataset.}
\end{table}

In the CIFAR10 dataset, our adaptive model achieved an end accuracy of 58.2\%, only marginally lower than the largest model (57.7\%) and significantly better than the catastrophic forgetting model (10\%). Despite the similar accuracies, our model required less than half the FLOPs needed by the largest model, making it significantly more efficient.

This pattern was consistent across all datasets. In each case, our adaptive model provided similar or better accuracy than the largest model while needing significantly fewer computational resources. Notably, in the case of MNIST, our model achieved an almost equivalent end accuracy (92.8\%) to the largest model (92.7\%), while requiring less than half the FLOPs (36\%).

\begin{table}[h!]
\centering
\begin{tabular}{lllll}
\hline
Model & End accuracy & Average accuracy over steps & Needed FLOPs \
\hline
Baseline & 98.8\% & 78.8\% & 100\% \
Largest model & 92.7\% & 76.9\% & 100\% \
Adaptive Model (ours) & 92.8\% & 76.1\% & 36\% \
Catastrophic forgetting & 60.1\% & 66.2\% & 100\% \
\hline
\end{tabular}
\caption{Performance comparison on MNIST dataset.}
\end{table}

In summary, our proposed method not only handles the inherent constraints of on-device training but also showcases efficient resource utilization while preserving model accuracy.


\subsection{Results}
The results of the above-mentioned experiments show that the presented method of incremental learning can be used to perform computations efficiently. The technique saves capacity at two points. The first is through an incremental approach, which is memory efficient since only a small fraction of the data set is stored. The second is that the model can grow with the task and therefore initially requires fewer resources in terms of computing and storage capacity.



\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over steps & Needed FLOPs \\
Baseline                & 85.4 \%        & 47.8 \%                      & 100 \%       \\
Largest model           & 57.7 \%        & 35.6 \%                      & 100 \%        \\
Adaptive Model          & 58.2 \%        & 35.9 \%                      & 43\%       \\
Catastrophic Forgotting & 10 \%        & 10 \%                      & 100 \%               
\end{tabular}%
}
\caption{CIFAR10 }
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs  \\
Baseline                & 55.3 \%        & 36.5 \%                      & 100 \%                     \\
Largest model           & 44.2 \%        & 28.9 \%                      & 100 \%                     \\
Adaptive Model          & 43.2 \%        & 26.1 \%                      & 49\%                       \\
Catastrophic Forgotting & 3.7 \%        & 3.6 \%                      & 100 \%                      
\end{tabular}%
}
\caption{CORe50 }

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs  \\
Baseline                & 95 \%        & 45.6 \%                      & 100 \%                       \\
Largest model           & 70.8 \%        & 35 \%                      & 100 \%                       \\
Adaptive Model          & 70.4 \%        & 33.7 \%                      & 36 \%                      \\
Catastrophic Forgotting & 3.8 \%        & 2.9 \%                      & 100 \%                      
\end{tabular}%
}
\caption{Spechcommands }

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs  \\
Baseline                & 98.8 \%        & 78.8 \%                      & 100 \%                     \\
Largest model           & 92.7 \%        & 76.9 \%                      & 100 \%                     \\
Adaptive Model          & 92.8 \%        & 76.1 \%                      & 36\%                       \\
Catastrophic Forgotting & 60.1 \%        & 66.2 \%                      & 100 \%                    
\end{tabular}%
}
\caption{MNIST }

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
                        & End accuracy & average accuracy over time & Needed FLOPs  \\
Baseline                & 83.1 \%        & 43.1 \%                      & 100 \%                     \\
Largest model           & 65.1 \%        & 37.3 \%                      & 100 \%                     \\
Adaptive Model          & 64.4 \%        & 36.9 \%                      & 36\%                       \\
Catastrophic Forgotting & 15 \%        & 12.5 \%                      & 100 \%                      
\end{tabular}%
}
\caption{HAR }
\end{table}



\subsubsection{Incremental learning}
With the presented technique, incremental learning can be successfully performed, as the experiments show. The advantage of using distilled datasets is the low memory overhead required to combat catastrophic forgetting. With only 1\% of the total size of the original dataset.



\subsubsection{Efficiencies of the adaptive model size}
A novelty of our technology is that the models can be expanded. By enlarging the models only when needed, instead of using a large model from the beginning, we save memory and computational resources. For example, our experiments have shown that with an adaptive model we only need 36\% of the FLOPS over the whole training process for speech commands and HAR, compared to a fixed model. With CIFAR10 we always need only 43\% of the FLOPs and even with a heavy data set like CORe50 we need only 49\% of the FLOPs. This saving is directly related to the energy saving and time saving. The experiments also show that the accuracy has little or no loss despite the large savings. Thus, in the best case, the CIFAR10 data set has a better average accuracy of 0.3 \% and the CORe50 data set has only an average loss of 2.8 \% accuracy over the whole training process.






==> Introger.tex <==
\section{Introduction} 

Problem vorstellen -> catastrophic forgetting\\

TinyML Vorstellen\\
restrictions TinyML\\

Lösung vorstellen:


Dataset distilation\\
TinyML brings computation and data storage closer to the origin of data.
TinyML bringt Machine learning (ML) näher zum Ursprung der Daten, in dem die ML-modelle direkt auf einem embedded gerät ausgeführt werden. 

In contrast to cloud servers, embedded systems are mostly very resource limited. Typical limitations in embedded devices  such as Micro-Controller Units (MCUs) are:

\begin{itemize} 
\item Limited device memory: for on-device training, we need to save more than just the weights and biases, e.g. also the activations and gradients.
\item Limited energy resources, e.g., due to being battery-powered: training requires complex calculations and, hence, more energy.
\item Limited computing power:  the device cannot run the training of the DNN in a given time.
\end{itemize}





The code for the algorithm is written in Python and is directly usable and available on GitHub: 




